DiffMoog: a Differentiable Modular Synthesizer for Sound Matching

This paper presents DiffMoog - a differentiable modular synthesizer with a comprehensive set of modules typically found in commercial instruments. Being differentiable, it allows integration into neural networks, enabling automated sound matching, to replicate a given audio input. Notably, DiffMoog facilitates modulation capabilities (FM/AM), low-frequency oscillators (LFOs), filters, envelope shapers, and the ability for users to create custom signal chains. We introduce an open-source platform that comprises DiffMoog and an end-to-end sound matching framework. This framework utilizes a novel signal-chain loss and an encoder network that self-programs its outputs to predict DiffMoogs parameters based on the user-defined modular architecture. Moreover, we provide insights and lessons learned towards sound matching using differentiable synthesis. Combining robust sound capabilities with a holistic platform, DiffMoog stands as a premier asset for expediting research in audio synthesis and machine learning.

==> 04_Implementation_Overview.tex <==
\section{Implementation Overview}

For clarity, we have aligned the nomenclature in this paper with the terms in our codebase. The code is organized as follows: Core implementation of the synthesizer is found under \texttt{src/synth}; Functionality of the sound matching system is at \texttt{src/model}; Operations related to dataset management housed in \texttt{src/dataset}; Configurations for training, synthesis, and loss functions are at the \texttt{configs} directory.

==> 06_System.tex <==
\section{End-to-End Sound Matching System}


